Stealing Training Graphs from Graph Neural Networks

Graph Neural Networks (GNNs) have shown promising results in modeling graphs in various tasks. The training of GNNs, especially on specialized tasks such as bioinformatics, demands extensive expert annotations, which are expensive and usually contain sensitive information of data providers. The trained GNN models are often shared for deployment in the real world. As neural networks can memorize the training samples, the model parameters of GNNs have a high risk of leaking private training data. Our theoretical analysis shows the strong connections between trained GNN parameters and the training graphs used, confirming the training graph leakage issue. However, explorations into training data leakage from trained GNNs are rather limited. Therefore, we investigate a novel problem of stealing graphs from trained GNNs. To obtain high-quality graphs that resemble the target training set, a graph diffusion model with diffusion noise optimization is deployed as a graph generator. Furthermore, we propose a selection method that effectively leverages GNN model parameters to identify training graphs from samples generated by the graph diffusion model. Extensive experiments on real-world datasets demonstrate the effectiveness of the proposed framework in stealing training graphs from the trained GNN.

==> 1_draft.tex <==
\section{Threat Model}
\textbf{Attacker's Goal.} 
Given a target classifier $f_{\theta} = p(y|\mathcal{G}): \mathcal{G}\xrightarrow{}\mathbf{P}^{C}$, which is trained on the private dataset $\mathcal{D}_{tar} = \{\mathcal{G}_i, y_i\}^{N_{tar}}_{i=1}$. $C$ is the number of the class on $\mathcal{D}_{tar}$.
The goal of the adversary in training graph stealing attack is to reconstruct the samples on the training data $\mathcal{D}_{tar}$. 
% generate graphs and make them as similar to the training graphs as possible 



% , the attacker aims to reconstruct samples on $\mathcal{D}_{tar}$.

\textbf{Attacker's Knowledge and Capability.}
We assume that the attacker has white-box access to $f_{\theta}$, which means that the attacker can access to the parameter $\theta$ of $f_{\theta}$. An public auxiliary dataset $\mathcal{D}_{aux}=\{\mathcal{G}_i, y_i\}^{N_{aux}}_{i=1}$ is available to the attacker.
$\mathcal{D}_{tar}$ lies in the low-dimensional manifold of $\mathcal{D}_{aux}$. 
Moreover, we also assume that a graph generator $g$ is available to the attacker.


% This assumption can help us to learn some basic common knowledge of the molecule graphs and reconstruct the training molecule graphs more effectively. In addition, we assume that the attacker 

\textbf{Problem Formulation}
This problem can be formulated as:
\begin{problem}
Given a target classifier $f_{\theta} = p(y|\mathcal{G}): \mathcal{G}\xrightarrow{}\mathbf{P}^{C}$, which is trained on the private dataset $\mathcal{D}_{tar} = \{\mathcal{G}_i, y_i\}^{N_{tar}}_{i=1}$. Given an public auxiliary dataset $\mathcal{D}_{aux}=\{\mathcal{G}_i, y_i\}^{N_{aux}}_{i=1}$, we aim to reconstruct $\mathcal{G}_{r}$ such that $\mathcal{G}_{r}$ is similar to $\mathcal{G}_{t}\in\mathcal{D}_{tar}$ by solving:
% \begin{equation}
% \begin{aligned}
%     \mathcal{G}_r&\in \mathcal{D}_{tar} \\
%     % \min_{\theta_{g}}~&{d(\mathcal{G}_{rec}, \mathcal{G}_{tar})}\\
%     s.t.~&\mathcal{G}_{r}=f_{g}(\mathcal{G}_{aux};|\mathcal{G}_{tar}|,y_{tar}, f_{\theta^*})\\
%     & \theta^* = \underset{\theta}{\arg\min}\sum_{\mathcal{G}_i\in\mathcal{D}_{tar}}l(f_{\theta}(\mathcal{G}_{i},y_{i}))\\
%     & \mathcal{G}_{aux} = \underset{\mathcal{G}\in\mathcal{D}_{aux}}{\arg\min}~l(f_{\theta^*}(\mathcal{G},y_{tar}))\\
% \end{aligned}
% \end{equation}
\begin{equation}
\begin{aligned}
    \max_{\theta_{g}}~|&{s(\mathcal{G}_{r}, \mathcal{G}_{t})}\\
    s.t.~&\mathcal{G}_{r}=f_{g}(\mathcal{G}_{a};|\mathcal{G}_{t}|,y_{t}, f_{\theta}),\\
    % & \theta^* = \underset{\theta}{\arg\min}\sum_{\mathcal{G}_i\in\mathcal{D}_{t}}l(f_{\theta}(\mathcal{G}_{i},y_{i})),\\
    % & \mathcal{G}_{a} = \underset{\mathcal{G}\in\mathcal{D}_{aux}}{\arg\min}~l(f_{\theta^*}(\mathcal{G},y_{t}))\\
    & \mathcal{G}_{t}\in\mathcal{D}_{tar},
\end{aligned}
\end{equation}
where $s(\cdot,\cdot)$ is to measure the similarity between two graphs. Both structural similarity and node feature similarity are involved. The details are introduced in Sec.~\ref{sec:evaluate_reconstruct_results}
\end{problem}
\section{Methodology}
In this section, we present the details of our method to reconstruct training graphs effectively. (Reconstruct training in optimization way)
\subsection{Reconstruct Training Graph }
In this subsection, we introduce the details of reconstructing training graph in optimization way. 

To reconstruct the graphs similar to the training graphs $\mathcal{G}_{t}\in\mathcal{D}_{tar}$,  we take the graphs in the auxiliary dataset $\mathcal{D}_{aux}$ and the target class $y_{t}$ as input. 
Specifically, we fix the number of nodes on the reconstructed graph as $n_r$, and select graphs from $\mathcal{D}_{aux}$ to reconstruct the graphs with $n_r$ based on the graphs select from $\mathcal{D}_{aux}$. 

Inspired from membership inference attacks~\cite{wu2021adapting}, the target classifier $f_{\theta}$ will classify its training data to its ground-truth class with a high confidence score while classifying the test data to its ground-truth class  with a relatively small confidence. Therefore, intuitively, if we choose a graph with a higher confidence score to the target class $y_t$, this graph would share more common properties to the training graphs of the class $y_t$ on $\mathcal{D}_{tar}$, which is more helpful for training graph reconstruction. The metric score of $\mathcal{G}_a$ on $\mathcal{D}_{aux}$ can be computed by
\begin{equation}
\begin{aligned}
m(\mathcal{G}_a) = -l(f_{\theta}(\mathcal{G}_a), y_t),
\end{aligned}
\end{equation}
where $l(\cdot,\cdot)$ is the cross entropy loss. After getting each graph's score, we select the graphs with top-$n$ highest scores in each class of $\mathcal{D}_{aux}$ as the candidate auxiliary graph set $\mathcal{D}_{ca}$ to reconstruct the training graph on $\mathcal{D}_{tar}$.

% Before reconstructing the traning graphs, we first modify 
% align the number of nodes on $\mathcal{G}_a$ with $n_r$. If $n_r > |\mathcal{G}_a|$, we inject $n_r-|\mathcal{G}_a|$ nodes to $\mathcal{G}_a$; If $n_r < |\mathcal{G}_a|$, we randomly drop $|\mathcal{G}_a|-n_r$ nodes from $\mathcal{G}_a$:
% \begin{equation}
% \begin{aligned}
%     \mathcal{G}_{a}' = m(\mathcal{G}_{a},n_r),
% \end{aligned}
% \end{equation}
% where $m(\mathcal{G}_{a},n_r)$ is the graph modification function to align the number of nodes on $\mathcal{G}_{a}$ based on the above rules.

Once the candidate auxiliary graphs set $\mathcal{D}_{ca}$ are determined, the next step is to reconstruct the training graphs on $\mathcal{D}_{tar}$.
We consider both graph structure and node features reconstructions. Given a $\mathcal{G} = ({A},{X})\in\mathcal{D}_{ca}$, $A\in\{0,1\}^{n\times n}$ and $D\in\mathbb{R}^{n\times d}$,
the reconstructed training graph $\hat{\mathcal{G}}=(\hat{{A}},\hat{{X}})$ is given by:
\begin{equation}
\label{eq:reconstruct_notation}
\begin{aligned}
    & \hat{{A}} = {A} + {C}\odot{S},~~~~{C}= \bar{{A}} - {{A}}, \\
    & \hat{{X}} = {{X}} + {Q},
\end{aligned}
\end{equation}
where $\odot$ is the element-wise product. ${Q}$ is the perturbation added on $X$ to reconstruct $\hat{{X}}$. $S\in\{0,1\}^{n\times n}$ is a boolean symmetric matrix to encode whether an edge in $\mathcal{G}$ is modified or not. If $s_{ij}=s_{ji}=1$, the edge between node $i$ and node $j$ is modified (add or remove edge). Otherwise, The edge is not modified if $i=j$ or $s_{ij}=0$.
The positive and negative entries on ${C}$ denote the edges are added to or removed from ${A}$, respectively. 

Training graph stealing attack can be mathematically formulated as an optimization problem:
\begin{equation}
\label{eq:group_membership_objective}
\begin{aligned}
\sum_{\mathcal{G}_i\in\mathcal{D}_{ca}}\min_{\hat{\mathcal{G}}_i\in\Phi{(\mathcal{G}_i)}}
l(f_{\theta}(\hat{\mathcal{G}}_i),y_i),
\end{aligned}
\end{equation}
where $l(\cdot,\cdot)$ is the cross entropy loss. $\Phi$ is the admissible space for reconstruction. This term indicates that we aim to find the training graphs $\hat{\mathcal{G}}_{i}$ that target classifier $f_{\theta}$ has minimal training loss on it. This insight is from membership inference attack that $f_{\theta}$ will classify its training data to its ground-truth class with a high confidence score.

To solve this optimization problem in Eq.~(\ref{eq:group_membership_objective}), we aim to seek ${S}_i$ and ${Q}_i$ in Eq.~(\ref{eq:reconstruct_notation}) for each graph $\mathcal{G}_i\in\mathcal{D}_{ca}$  to minimize the training loss on the ground-truth label
the problem can be reformulated into:
\begin{equation}
\begin{aligned}
&\sum_{\mathcal{G}_i\in\mathcal{D}_{ca}}\min_{\mathbf{s}_i,\mathbf{q}_i}h(\mathbf{s}_i,\mathbf{q}_i,\theta,\mathcal{G}_i,y_i) \\
= & \sum_{\mathcal{G}_i\in\mathcal{D}_{ca}}\min_{\mathbf{s}_i,\mathbf{q}_i}l(f_{\theta}(\hat{\mathcal{G}}_i),y_i),\\
\end{aligned}
\end{equation}
where $\mathbf{s}_i\in\{0,1\}^{\bar{n}}$ and $\mathbf{q}_i\in\mathbb{R}^{n\times{d}}$ are the vector-form of $S_i$ and $Q_i$, respectively. Especially, $\mathbf{s}_i$ consists of $\bar{n}:=n(n-1)/2$ unique variable on $S_i$.

Due to the discreteness of graph data, for the each of optimization, we then relax $\mathbf{s}\in\{0,1\}^{\bar{n}}$ to its convex hull $\mathbf{s}\in[0,1]^{\bar{n}}$ and view it as a continuous optimization. Then we apply the projected gradient descent (PGD) to use the gradient of w.r.t. $\mathbf{s}_{i}$ to minimize $h(\mathbf{s}_i,\mathbf{q}_i,\theta,\mathcal{G}_i,y_i)$:
\begin{equation}
\begin{aligned}
    &\mathbf{s}^{(t)}_{i} = \Pi_{\mathcal{S}}\left[\mathbf{s}^{(t-1)}_{i} - \beta\cdot \nabla_{\mathbf{s}^{(t-1)}_{i}}h(\mathbf{s}_i,\mathbf{q}_i,\theta,\mathcal{G}_i,y_i)\right],\\
    &\mathbf{q}^{(t)}_{i} = \Pi_{\mathcal{Q}}\left[\mathbf{q}^{(t-1)}_{i} -\mu\cdot \nabla_{\mathbf{q}^{(t-1)}_{i}}h(\mathbf{s}_i,\mathbf{q}_i,\theta,\mathcal{G}_i,y_i)\right],
\end{aligned}
\end{equation}
where $\mathbf{s}^{(t)}_{i}$ and $\mathbf{q}^{(t)}_{i}$ are the optimization results after updating $t$ steps. $\beta$ and $\mu$ are the learning rates for $\mathbf{s}$ and $\mathbf{q}$, respectively.
$\Pi_{\mathcal{S}}(\mathbf{a}):=\underset{\mathbf{s}\in\mathcal{S}}{\arg\min}||\mathbf{s}-\mathbf{a}||_{2}^{2}$ is the projection vector at $\mathbf{a}$, where $\mathcal{S} = \{\mathbf{s}|\mathbf{s}\in[0,1]^{\bar{n}}\}$. $\Pi_{\mathcal{Q}}(\mathbf{a}):= \underset{\mathbf{a}\in\mathcal{Q}}{\arg\min}||\mathbf{q}-\mathbf{a}||^2_2$. $\mathcal{Q}$ depends on the feature properties of the dataset. 

To further power the effectiveness of training graph stealing, inspired from~\cite{haim2022reconstructing}, we have the insight that 
the parameter $\theta$ of target classifier $f_{\theta}$ are a linear combinations of the derivatives of the networks at the training data points. For the binary class dataset, we consider the following objectives:
\begin{equation}
\label{eq:loss_stationary}
\begin{aligned}
\mathcal{L}_{\text{stationary}}(\hat{\mathcal{G}}_{1},\cdots,\hat{\mathcal{G}}_{m},\lambda_1,\cdots,\lambda_{m})
& = ||\theta - \sum_{i=1}^{m}[\lambda_{i} y_{i}\nabla_{\theta}f_{\theta}(\hat{\mathcal{G}}_i)]||_{2}^{2}, \\
\mathcal{L}_{\lambda}(\lambda_1,\cdots,\lambda_m) & = \sum_{i=1}^{m}\max\{-\lambda_i,0\},
\end{aligned}
\end{equation}

For multi-class dataset, we can redefine $y_{i}\nabla_{\theta}f_{\theta}(\hat{\mathcal{G}}_i)$ as the the difference between the classification score for the true label and the maximum score for the other labels, therefore, the objectives in Eq.~(\ref{eq:loss_stationary}) can be rewrote as:
\begin{equation}
\label{eq:loss_stationary_multi}
\begin{aligned}
\mathcal{L}_{\text{stationary}}(\hat{\mathcal{G}}_{1},\cdots,\hat{\mathcal{G}}_{m},\lambda_1,\cdots,\lambda_{m})
& = ||\theta - \sum_{i=1}^{m}[\lambda_{i} \nabla_{\theta}(f_{\theta, y_{i}}(\hat{\mathcal{G}}_i) - \max_{j\neq{y_i}}f_{\theta, j}(\hat{\mathcal{G}}_i))]||_{2}^{2}, \\
\mathcal{L}_{\lambda}(\lambda_1,\cdots,\lambda_m) & = \sum_{i=1}^{m}\max\{-\lambda_i,0\},
\end{aligned}
\end{equation}

Therefore, the overall objective function is:
\begin{equation}
\begin{aligned}
\mathcal{L}_{ce} = \sum_{\mathcal{G}_i\in\mathcal{D}_{ca}}\min_{\hat{\mathcal{G}}_i\in\Phi{(\mathcal{G}_i)}}
l(f_{\theta}(\hat{\mathcal{G}}_i),y_i)\\
\mathcal{L} = \mathcal{L}_{ce} + \sigma_1\cdot\mathcal{L}_{\text{stationary}} + \sigma_2\cdot\mathcal{L}_{\lambda}
\end{aligned}
\end{equation}
% \subsection{Questions}
% Remaining questions:
% \begin{itemize}
%     % \item Do we need to specify the constraints in the optimization formula?
%     \item Increase the size of $\mathcal{D}_{ca}$ may make the optimization harder
% \end{itemize}
\section{Evaluation}
\subsection{Experimental Setup}
\textbf{Baselines.} We consider the following methods as baseline:
\begin{itemize}
    \item Random Graphs: We use Erdos-Renyi (ER) model to randomly generate the reconstructed graph connections and the node features are randomly sampled from $\mathcal{D}_{aux}$
    \item Sample graphs with lowest loss to the true labels in $\mathcal{D}_{aux}$ as the reconstructed graphs. 
    \item GraphMI~\cite{zhang2021graphmi}: We modify the GraphMI to fit into our tasks. Specifically, we randomly select some auxiliary graphs and apply GraphMI to this graph to reconstruct graph.
    \item 

\end{itemize}

\section{Threat Model}
\subsection{Problem Definition}
Given a target classifier $f_{\theta} = p(y|\mathcal{G}): \mathcal{G}\xrightarrow{}\mathbf{P}^{C}$, which is trained on the private dataset $\mathcal{D}_{tar} = \{\mathcal{G}_i, y_i\}^{N_{tar}}_{i=1}$, the attacker aims to reconstruct samples on $\mathcal{D}_{tar}$.

\subsection{Attacker Knowledge}
We assume that the attacker has white-box access to $f_{\theta}$, which means that the attacker can access to the parameter $\theta$ of $f_{\theta}$. Moreover, we assume that an public auxiliary dataset $\mathcal{D}_{aux}=\{\mathcal{G}_i, y_i\}^{N_{aux}}_{i=1}$ is available to the attacker, which share some common rules with the private dataset. In other words, the private dataset lies in the low dimensional manifold of shadow dataset. This assumption can help us to learn some basic common knowledge of the molecule graphs and reconstruct the training molecule graphs more effectively. 

\section{Methodology}
Recall that the goal of attackers is to reconstruct the samples on $\mathcal{D}_{tar}$, we can reformalize this problem into two steps. The first step is to approximate the distribution $p_{tar}(\mathcal{G}|y)$. The second step is to generate graph $\mathcal{G}$ based on the approximated distribution $\bar{p}_{tar}(\mathcal{G}|y)$ such that $\mathcal{G}$ is on $\mathcal{D}_{tar}$. 

\paragraph{Key steps}
\begin{itemize}
    \item Train a common generator $p_{G}(\mathcal{G}|\mathbf{z})$ on $D_{aux}$.
    \item Learn the target posterior $p_{tar}(\mathcal{G})$ with an approximated distribution $q(\mathcal{G})$ by optimizing Eq.(\ref{q_star_z_upper_bound_replace_with_aux}).
    \item Add some constraints to     
\end{itemize}

\subsection{Approximate Target Distribution}
We formulate the training stealing attack as the variational inference~\cite{wang2021variational}. To reconstruct the sample on $\mathcal{D}_{tar}$, we first need to approximate the class conditional distribution $p_{tar}(\mathcal{G}|y)$, which can be represented by a variational distribution $q(\mathcal{G})\in Q_{\mathcal{G}}$. 
$Q_{\mathcal{G}}$ is the variational family, which contains all distribution that lie on the manifold of $p_{tar}(\mathcal{G})$ and $p_{aux}(\mathcal{G})$. 
We can achieve it by optimizing the following objectives:
\begin{equation}
\label{q_star_G}
\begin{aligned}
    q^*(\mathcal{G}) & = \underset{q\in Q_{\mathcal{G}}}{\arg\min}\{D_{KL}(q(\mathcal{G}||p_{tar}(\mathcal{G}|y)))\} \\
    & = \underset{q\in Q_{\mathcal{G}}}{\arg\min}\{\mathbb{E}_{q(\mathcal{G})}[-\log{p_{tar}(y|\mathcal{G})}]+D_{KL}(q(\mathcal{G})||p_{tar}(\mathcal{G})))\}
\end{aligned}
\end{equation}

To minimize Eq.~(\ref{q_star_G}), we need to compute $D_{KL}(q(\mathcal{G}||p_{tar}(\mathcal{G})))$. However, the true graph prior $p_{tar}(\mathcal{G})$ is not accessible. Therefore, we use the auxiliary dataset $D_{aux}$ to learn the graph prior $p_{aux}(\mathcal{G})$ by training a common generator $p_{G}(\mathcal{G}|\mathbf{z})$. The choices of common generators can be GAN or graph diffusion, etc. For simplicity, we initially choose GAN~\cite{de2018molgan} as the generator.


For the common generator, we make the following assumption~\cite{wang2021variational}: The manifold of latent vector $\mathbf{z}$ of the common generator $p_{G}(\mathcal{G}|\mathbf{z})$ trained on $\mathcal{D}_{aux}$ covers the latent vector of the training data $\mathcal{D}_{tar}$. In other words, there exists a target prior $p_{tar}{(\mathbf{z})}$, which is possibly different from $p_{aux}{(\mathbf{z})}$, such that $p_{tar}{(\mathcal{G})}\approx\mathbb{E}_{p_{tar}(\mathbf{z})}[p_{G}(\mathcal{G}|\mathbf{z})]$. Therefore, this problem can be transferred from learning the approximated true target posterior with a variational distribution $q(\mathcal{G})$ to $q(\mathbf{z})$. (For example, $p_{aux}(\mathcal{G})$ could be the distribution of representative drugs for all diseases, while $p_{tar}$ could be the distribution of drugs for a specific disease.)

Then we can approximate the objectives of Eq.~(\ref{q_star_G}) with 
\begin{equation}
\label{q_star_z}
\begin{aligned}
    q^*(\mathbf{z}) = \underset{q\in Q_{\mathcal{G}}}{\arg\min}\{\mathbb{E}_{\mathbf{z}\sim q(\mathbf{z})}[-\log{p_{tar}(y|p_{G}(\mathcal{G}|\mathbf{z}))}]+D_{KL}(\mathbb{E}_{q(\mathbf{z})}[p_{G}(\mathcal{G}|\mathbf{z})]||\mathbb{E}_{p_{tar}(\mathbf{z})}[p_{G}(\mathcal{G}|\mathbf{z})])\}
\end{aligned}
\end{equation}

According to Proposition 1 in~\cite{wang2021variational}, we have 
\begin{equation}
\label{proposition_1_VMI}
D_{KL}(q(\mathbf{z})||p_{tar}(\mathbf{z}))>D_{KL}(\mathbb{E}_{q(\mathbf{z})}[p_{G}(\mathcal{G}|\mathbf{z})]||\mathbb{E}_{p_{tar}(\mathbf{z})}[p_{G}(\mathcal{G}|\mathbf{z})]),
\end{equation}
the upper bound of Eq.(\ref{q_star_z}) is then obtained:
\begin{equation}
\label{q_star_z_upper_bound}
\begin{aligned}
q^*(\mathbf{z}) = \underset{q\in Q_{\mathcal{G}}}{\arg\min}\{\mathbb{E}_{\mathbf{z}\sim q(\mathbf{z})}[-\log{p_{tar}(y|p_{G}(\mathcal{G}|\mathbf{z}))}]+D_{KL}(q(\mathbf{z})||p_{tar}(\mathbf{z}))\}.
\end{aligned}
\end{equation}

Since we do not have the access to $p_{tar}(\mathbf{z})$, to optimize Eq.(\ref{q_star_z_upper_bound}), we replace it with $p_{aux}(\mathbf{z})$. 
The final objective function is:
\begin{equation}
\label{q_star_z_upper_bound_replace_with_aux}
\begin{aligned}
q^*(\mathbf{z}) = \underset{q\in Q_{\mathcal{G}}}{\arg\min}\{\mathbb{E}_{\mathbf{z}\sim q(\mathbf{z})}[-\log{p_{tar}(y|p_{G}(\mathcal{G}|\mathbf{z}))}]+D_{KL}(q(\mathbf{z})||\gamma p_{aux}(\mathbf{z}))\},
\end{aligned}
\end{equation}
where $gamma$ is a power coefficient to prevent the classifier from over- or under-confident.
